PowerAlert: An Integrity Checker using Power Measurement

We propose PowerAlert, an efficient external integrity checker for untrusted hosts. Current attestation systems suffer from shortcomings in requiring complete checksum of the code segment, being static, use of timing information sourced from the untrusted machine, or use of timing information with high error (network round trip time). We address those shortcomings by (1) using power measurements from the host to ensure that the checking code is executed and (2) checking a subset of the kernel space over a long period of time. We compare the power measurement against a learned power model of the execution of the machine and validate that the execution was not tampered. Finally, power diversifies the integrity checking program to prevent the attacker from adapting. We implement a prototype of PowerAlert using Raspberry pi and evaluate the performance of the integrity checking program generation. We model the interaction between PowerAlert and an attacker as a game. We study the effectiveness of the random initiation strategy in deterring the attacker. The study shows that \power forces the attacker to trade-off stealthiness for the risk of detection, while still maintaining an acceptable probability of detection given the long lifespan of stealthy attacks.

==> data.tex <==
%How to get the training data (estimate the time needed)
%Will a high-level frequency analysis aid
The goal is to find out what is normal timing for the calls and what is the normal shape of the power signal. PowerAlert is initialized at the beginning of the operation of the untrusted machine.
\subsection{Timing Analysis}
To find the timing needed for each operation we have to methods:
\begin{enumerate}
\item Find the instructions to find each process and then use the latency/instruction to find the total number of cycles per process. This has to be done for each kernel version, and compiler. The time needed for each process becomes the frequency of the processor multiplied by the number of cycles.
\item Assume that the system is secure and then compute a baseline. The baseline is the average time needed to run the instrumentation script.
\end{enumerate}

==> pa1.tex <==
\begin{msc}{Example}
\declinst{prover}{}{Prover}
\declinst{verifier}{}{Verifier}
\mess{Start PA-proto}{verifier}{prover}
\nextlevel
\action*{%
\begin{minipage}{3cm}\centering 
run \texttt{x = ls /proc/}
\end{minipage}%
}{prover}
\nextlevel[4]
\mess{Send $x$}{prover}{verifier}
\nextlevel
\action*{%
\begin{minipage}{3cm}\centering
Choose a random number and key\\
$r\in\{0,1\}^*, k\in\{0,1\}^*$
\end{minipage}}{verifier}
\nextlevel[5]
\mess{Send $r,k$}{verifier}{prover}
\nextlevel
\action*{%
\begin{minipage}{3cm}\centering
fork $r$ process \\
run \texttt{rs = ls /proc} k times \\
m = encrypt \texttt{rs} with $k$
\end{minipage}}{prover}
\nextlevel[6]
\mess{Send $m$}{prover}{verifier}
\nextlevel
\action*{%
\begin{minipage}{3cm}\centering
verify \texttt{m} \\
correlate with power
\end{minipage}}{verifier}
\nextlevel[2]
\end{msc}

==> pa2.tex <==
\begin{msc}{PowerAlert-Protocol}
\declinst{prover}{}{Prover}
\dummyinst{j}
\declinst{verifier}{}{Verifier}

\mess{Init \power-protocol}{verifier}{prover}
\nextlevel

\action*{%
\begin{minipage}{3cm}\centering
Choose random\\
$\mathcal{L}\in\{0,1\}^*, \eta\in\{0,1\}^*, f\in\mathcal{P}$
\end{minipage}}{verifier}

\nextlevel[3]
\action*{%
\begin{minipage}{3cm}\centering
record $i(t)$
\end{minipage}}{verifier}
\mess*{}{verifier}{prover}
\nextlevel[3]

\mess{$<\mathcal{L},\eta,f>$}{verifier}{prover}
\nextlevel


\action*{%
\begin{minipage}{3cm}\centering
$y=f(\mathcal{L},\eta,x)$
\end{minipage}}{prover}

\nextlevel[2]
\mess{$<y>$}{prover}{verifier}
\nextlevel

\action*{%
\begin{minipage}{3cm}\centering
\begin{enumerate}
\item stop $i(t)$
\item verify $<y>$
\item validate $i(t)$
\end{enumerate}
\end{minipage}}{verifier}
\nextlevel[3]
\end{msc}

==> psfmc.tex <==
\begin{tikzpicture}[scale=0.2]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (28.2,-21.3) circle (3);
\draw (28.2,-21.3) node {$S_0$};
\draw [black] (28.2,-21.3) circle (2.4);
\draw [black] (12.5,-21.3) circle (3);
\draw (12.5,-21.3) node {$S_1$};
\draw [black] (43.4,-21.3) circle (3);
\draw (43.4,-21.3) node {$S_2$};
\draw [black] (25.822,-23.114) arc (-60.41313:-119.58687:11.083);
\fill [black] (14.88,-23.11) -- (15.33,-23.94) -- (15.82,-23.07);
\draw (20.35,-25.06) node [below] {$network$};
\draw [black] (15.331,-20.316) arc (104.79191:75.20809:19.658);
\fill [black] (25.37,-20.32) -- (24.72,-19.63) -- (24.47,-20.6);
\draw [black] (41.168,-23.288) arc (-57.02467:-122.97533:9.863);
\fill [black] (41.17,-23.29) -- (40.23,-23.3) -- (40.77,-24.14);
\draw (35.8,-25.38) node [below] {$hash$};
\draw [black] (30.965,-20.147) arc (107.34327:72.65673:16.22);
\fill [black] (30.96,-20.15) -- (31.88,-20.39) -- (31.58,-19.43);
\draw [black] (26.877,-18.62) arc (234:-54:2.25);
\draw (28.2,-14.05) node [above] {$idle$};
\fill [black] (29.52,-18.62) -- (30.4,-18.27) -- (29.59,-17.68);
\end{tikzpicture}
